YOLO-ReT: Towards High Accuracy Real-time Object Detection on Edge GPUs

Performance of object detection models has been growing rapidly on two major fronts, model accuracy and efficiency. However, in order to map deep neural network (DNN) based object detection models to edge devices, one typically needs to compress such models significantly, thus compromising the model accuracy. In this paper, we propose a novel edge GPU friendly module for multi-scale feature interaction by exploiting missing combinatorial connections between various feature scales in existing state-of-the-art methods. Additionally, we propose a novel transfer learning backbone adoption inspired by the changing translational information flow across various tasks, designed to complement our feature interaction module and together improve both accuracy as well as execution speed on various edge GPU devices available in the market. For instance, YOLO-ReT with MobileNetV2x0.75 backbone runs real-time on Jetson Nano, and achieves 68.75 mAP on Pascal VOC and 34.91 mAP on COCO, beating its peers by 3.05 mAP and 0.91 mAP respectively, while executing faster by 3.05 FPS. Furthermore, introducing our multi-scale feature interaction module in YOLOv4-tiny and YOLOv4-tiny (3l) improves their performance to 41.5 and 48.1 mAP respectively on COCO, outperforming the original versions by 1.3 and 0.9 mAP.

==> tables/devices.tex <==
\begin{table*}[]
\footnotesize
\begin{center}
% \setlength\tabcolsep{4pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
& \multicolumn{2}{|c|}{\textbf{Desktop GPU}} & \multicolumn{3}{|c|}{\textbf{Edge GPU Devices}} & \multicolumn{2}{|c|}{\textbf{Edge Non-GPU Devices}} \\
% \hline
\cline{2-8}
 & \textbf{Tesla P100} & \textbf{Tesla V100} & \textbf{Jetson Nano} & \textbf{Jetson NX} & \textbf{Jetson AGX} & \textbf{Raspberry Pi 4} & \textbf{Tinker Edge T} \\
\hline

\textbf{Architecture} & Pascal GPU & Volta GPU & Maxwell GPU & Volta GPU & Volta GPU & VideoCore VI & Edge TPU \\
\textbf{CUDA Cores} & 3584 cores & 5120 cores & 128 cores & 384 cores & 512 cores & -- & -- \\
\textbf{Memory} & 16 GB & 16 GB & 4 GB & 8 GB & 32 GB & 1 GB & 1 GB \\
\textbf{Performance (FP16)} & 9.53 TFLOPs & 14.13 TFLOPs & 472 GFLOPs & 6 TFLOPs & 11 TFLOPs & 32 GFLOPs & 4 TOPs \\
\textbf{Performance (INT8)} &  &  & -- & 21 TOPs & 32 TOPs & 32 GFLOPs & 4 TOPs \\
\textbf{Power} & & & & & & & \\
\textbf{Cost (?)} & \$7,374 & \$10,664 & \$99 & \$399 & \$999 & \$35 & \$168 \\
\hline

\end{tabular}
\end{center}

\caption{Comparison of theoretical computing power provided by various devices. {\color{red} (David: This table looks outdated. Nano has two versions: 4GB and 2GB. AGX has 32GB memory and a much lower price now. TX2 is dead and replaced by NX. For desktops, P100 is old and there's A100. V100 has 32GB memory. For non-GPU devices, there is OpenCV AI Kit (OAK).)}}\label{tab:devices}
\end{table*}

